On Calogero-Moser cellular characters for imprimitive complex reflection groups

We study the relationship between Calogero-Moser cellular characters and characters defined from vectors of a Fock space of type $A_{\infty}$. Using this interpretation, we show that Lusztig's constructible characters of the Weyl group of type $B$ are sums of Calogero-Moser cellular characters. We also give an explicit construction of the character of minimal $b$-invariant of a given Calogero-Moser family of the complex reflection group $G(l,1,n)$.

==> sections/CMinclude.tex <==

%\begin{abstract}

%\end{abstract}



%\tableofcontents
\section{Computation of certain monomial elements}

Let $l\in \mathbb{N}_{>0}$ and let ${\bf s}=(s_1,\ldots,s_l) \in \mathbb{Z}^l$ be such that 
$$s_1\leq s_2 \leq \ldots  \leq s_l$$
Let ${\bf \lambda}=(\lambda^1,\ldots,\lambda^l)$ be an $l$-partition of rank $n\in \mathbb{N}$ and consider its associated ${\bf s}$-symbol 

  $${\bf S}=\left(\begin{array}{cccccccc}
\beta_1^l & \beta_2^l & \ldots  &\beta_{s_1+m}^l &   \ldots &  \beta_{s_2+m}^l & \ldots & \beta_{s_l+m}^l  \\
\ldots& \ldots &\ldots &\ldots & \ldots & \ldots   \\
\beta_1^2 &\beta_2^2&\ldots &\beta_{s_1+m}^2   &    \ldots & \beta_{s_2+m}^2\\
 \beta_1^1& \beta_2^1 &\ldots &  \beta_{s_1+m}^1 & &\\
\end{array}
\right)$$
where $m\in \mathbb{N}$ is a sufficiently large integer. 

Now, we say that the  $l$-partition ${\bf \lambda}$ is a simple $l$-partition if the associated symbol satisfies 
$$\beta_1^l\leq \ldots \beta_1^l\leq \beta_2^l\leq \ldots \leq \beta_2^1 \leq \ldots \leq \beta_{s_1+m}^l  \leq \ldots \leq \beta_{s_1+m}^1  \leq \beta_{s_2+m}^l \leq \ldots \leq  \beta_{s_2+m}^2\leq \ldots 
\leq \beta_{s_l+m}^l \leq \ldots $$
that is it decreased from top to bottom and left to right. The associated symbol is then standard.  Note that in each block (and in each CM family) there exist one unique simple $l$-partition. 


Let 
$$\sigma=(\sigma_1,\sigma_2,\ldots,\sigma_{s_l+m})\in (\mathfrak{S}_{l})^{s_1+m} \times (\mathfrak{S}_{l-1})^{s_2-s_1}\times \ldots \times (\mathfrak{S}_{1})^{s_l-s_{l-1}}$$ 
We say that $\sigma$ is admissible for the symbol ${\bf S}$ if 
\begin{itemize}
\item the element 
  $${\bf S}^{\sigma}=\left(\begin{array}{cccccccc}
\beta_1^{\sigma_1(l)} & \beta_2^{\sigma_2 (l)} & \ldots  &\beta_{s_1+m}^{\sigma_{s_1+m} (l)} &   \ldots &  \beta_{s_2+m}^{\sigma_{s_2+m} (l)} & \ldots & \beta_{s_l+m}^{\sigma_{s_l+m} (l)}  \\
\ldots& \ldots &\ldots &\ldots & \ldots & \ldots   \\
\beta_1^{\sigma_1 (2)} &\beta_2^{\sigma_2 (2)}&\ldots &\beta_{s_1+m}^{\sigma_{s_1+m} (2) }  &    \ldots & \beta_{s_2+m}^{\sigma_{s_2+m} (2)}\\
 \beta_1^{\sigma_1 (1)}& \beta_2^{\sigma_2 (1) }&\ldots &  \beta_{s_1+m}^{\sigma_{s_1+m} (1) } & &\\
\end{array}
\right)$$
is such that  each row of the above symbol has no repetitions. 
\item $\sigma$ has minimal length towards all the  $w \in  (\mathfrak{S}_{l})^{s_1+m} \times (\mathfrak{S}_{l-1})^{s_2-s_1}\times \ldots \times (\mathfrak{S}_{1})^{s_l-s_{l-1}} $ such that  ${\bf S}^{\sigma}={\bf S}^{w}$
\end{itemize}
We denote by $\mathfrak{S} (S)$ the set of admissible 
 elements in $(\mathfrak{S}_{l})^{s_1+m} \times (\mathfrak{S}_{l-1})^{s_2-s_1}\times \ldots \times (\mathfrak{S}_{1})^{s_l-s_{l-1}}$. 
 If $\sigma \in  \mathfrak{S} (S)$, then ${\bf S}^{\sigma}$ 
  is  the symbol of an $l$-partition of rank $n$ that we denote by ${\bf \lambda}^{\sigma}$. 

Now if we fix $\sigma \in   \mathfrak{S} (S)$ and an associated admissible symbol ${\bf S}^{\sigma}$, we define the following number 
$$M({\bf S}^{\sigma})=\sum_{j=2,\ldots,s_l+m} \sum_{t\leq l }     \sharp \{ k>t \ |\ \beta_{j-1}^{\sigma_{j-1} (k)} =\beta_j^{\sigma_j (t)} \}$$

\begin{prop}
Let ${\bf \lambda}$ be a simple $l$-partition.  Consider the monomial bases $A({\bf \lambda})$ defined in \cite{GJ}. Then we have 
$$A({\bf \lambda})= \sum v^{ N(\sigma,{\bf \lambda}) }  {\bf \lambda}^{\sigma}$$
where the sum is on all $\sigma=(\sigma_1,\sigma_2,\ldots,\sigma_{s_l+m})\in    \mathfrak{S} (S)$ and where 
$$N(\sigma,{\bf \lambda})=l(\sigma)-M({\bf S}^{\sigma})$$

\end{prop}


Here is an example, the number of admissible symbols must be : $1 \times 1\times 1 \times 1 \times \left( \begin{array}{c}  2 \\ 3\end{array}\right) \times 2 \times 1 \times 1 \times 1 \times \left( \begin{array}{c}  2 \\ 3\end{array}\right) \times 1=18$
\begin{verbatim}
1.v^0
[ 0, 1, 2, 4, 5, 7 ]
[ 0, 2, 3, 5 ]
[ 1, 2, 4 ]
[ 1, 2, 4 ]
2.v (One permutation on the 3rd row : s_2 on c_3)
[ 0, 1, 2, 4, 5, 7 ]
[ 0, 2, 4, 5 ]
[ 1, 2, 3 ]
[ 1, 2, 4 ]
3.v^2 (s_1.s_2 on c3)
[ 0, 1, 2, 4, 5, 7 ]
[ 0, 2, 4, 5 ]
[ 1, 2, 4 ]
[ 1, 2, 3 ]
4.v (s_2 on c1)
[ 0, 1, 2, 4, 5, 7 ]
[ 1, 2, 3, 5 ]
[ 0, 2, 4 ]
[ 1, 2, 4 ]
5.v^2 (s_2 on c1 and c_2 on c3) 
[ 0, 1, 2, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 0, 2, 3 ]
[ 1, 2, 4 ]
6.v^3 (s_2 on c1, s_1 s_2 on c3)
[ 0, 1, 2, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 0, 2, 4 ]
[ 1, 2, 3 ]
7.v^2 (s_2s_1 on c1)
[ 0, 1, 2, 4, 5, 7 ]
[ 1, 2, 3, 5 ]
[ 1, 2, 4 ]
[ 0, 2, 4 ]
8.v^3 (s_2s_1 on c1, s_2 on c3)
[ 0, 1, 2, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 1, 2, 3 ]
[ 0, 2, 4 ]
9.v^4 (s_2s_1 on c1, s_2 s_1 on c3)
[ 0, 1, 2, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 1, 2, 4 ]
[ 0, 2, 3 ]
10.v (s_3 on c2 s_3 on c3 minus 1 
(one integer 2 on c2 ``above'' the 2 on c3))
[ 0, 2, 3, 4, 5, 7 ]
[ 0, 1, 2, 5 ]
[ 1, 2, 4 ]
[ 1, 2, 4 ]
11.v^2 (s_2 s_3 on c_1, s_3 on c2  minus 2
 (one integer 2 on c2 ``above'' the 2 on c3 AND one integer 1 on c1 ``above'' the 1 on c2))
[ 1, 2, 3, 4, 5, 7 ]
[ 0, 1, 2, 5 ]
[ 0, 2, 4 ]
[ 1, 2, 4 ]
12.v^3 (s_2s_3s_1 on c1, s_3 on c2 , s_3 on c3  minus 2 
(one integer 2 on c2 ``above'' the 2 on c3 AND one integer 1 on c1 ``above'' the 1 on c2))
[ 1, 2, 3, 4, 5, 7 ]
[ 0, 1, 2, 5 ]
[ 1, 2, 4 ]
[ 0, 2, 4 ]
13.v^2  (s_1 on c1, s_3s_2 on c2, s_3s_2 on c2   minus 3
 (two integers 2 on c2 ``above'' the 2 on c3  AND one integer 1 on c1 ``above'' the 1 on c2))
[ 0, 2, 3, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 0, 1, 2 ]
[ 1, 2, 4 ]
14.v^3 (s_2 s_3 on c1 s_2 s_3 on c2 s_2 s_3 on c3 minus 3 
(two integers 2 on c2 ``above'' the 2 on c3  AND one integer 1 on c1 ``above'' the 1 on c2))
[ 1, 2, 3, 4, 5, 7 ]
[ 0, 2, 4, 5 ]
[ 0, 1, 2 ]
[ 1, 2, 4 ]
15.v^4 (s_2 s_3s_1s_2 on c1 s_2 s_3 on c2 s_2 s_3 on c3 minus 4 
(two integers 2 on c2 ``above'' the 2 on c3 AND two integer 1 on c1 ``above'' the 1 on c2))
[ 1, 2, 3, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 0, 1, 2 ]
[ 0, 2, 4 ]
16.v^3 (s_2s_1 on c1, s_3 s_2 s_1 on c2, s_3 s_2 s_1 on c3 minus 5 
(three integers 2 on c2 ``above'' the 2 on c3 AND two integer 1 on c1 ``above'' the 1 on c2))
[ 0, 2, 3, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 1, 2, 4 ]
[ 0, 1, 2 ]
17.v^4  (s_2s_3s_1 on c1,s_3 s_2 s_1 on c2, s_3 s_2 s_1 on c3 minus 5
 (three integers 2 on c2 ``above'' the 2 on c3 AND two integer 1 on c1 ``above'' the 1 on c2))
[ 1, 2, 3, 4, 5, 7 ]
[ 0, 2, 4, 5 ]
[ 1, 2, 4 ]
[ 0, 1, 2 ]
18.v^5  (s_2 s_3s_1s_2 on c1 s_3 s_2 s_1 on c2, s_3 s_2 s_1 on c3 minus 5
 (three integers 2 on c2 ``above'' the 2 on c3 AND two integer 1 on c1 ``above'' the 1 on c2))
[ 1, 2, 3, 4, 5, 7 ]
[ 1, 2, 4, 5 ]
[ 0, 2, 4 ]
[ 0, 1, 2 ]
\end{verbatim}

Another example :
\begin{verbatim}
1.v^0
[ 0, 1, 3, 4, 7 ]      5.   6
[ 0, 2, 3, 5, 8 ]      6.  5
[ 0, 3, 4, 6 ]          7.  7
[ 1, 3, 4, 7 ].        4.  4
\end{verbatim}
gives $2\times 3 \times 3! \times 3 \times 2 \times 3 = 648$ elements. 
\begin{verbatim}
527.v^6
[ 0, 2, 3, 6, 7 ]
[ 0, 3, 4, 7, 8 ]
[ 1, 3, 4, 5 ]
[ 0, 1, 3, 4 ]
\end{verbatim}
$s_1$ on $c_1$, $s_1 s_2 s_3$ on $c_2$,  $s_1 s_2$ on $c_3$, $s_2 s_3 s_1 s_2 s_3$ on $c_4$ : so the length is $11$ minus $5$ (because $2$ numbers $4$ above the $4$ in row $4$,
 two $3$ above the $3$ in row $3$ and one $1$ above the $1$ in row $2$). 






